AgriCLIP: Adapting CLIP for Agriculture and Livestock via Domain-Specialized Cross-Model Alignment

Capitalizing on vast amount of image-text data, large-scale vision-language pre-training has demonstrated remarkable zero-shot capabilities and has been utilized in several applications. However, models trained on general everyday web-crawled data often exhibit sub-optimal performance for specialized domains, likely due to domain shift. Recent works have tackled this problem for some domains (e.g., healthcare) by constructing domain-specialized image-text data. However, constructing a dedicated large-scale image-text dataset for sustainable area of agriculture and livestock is still open to research. Further, this domain desires fine-grained feature learning due to the subtle nature of the downstream tasks (e.g, nutrient deficiency detection, livestock breed classification). To address this we present AgriCLIP, a vision-language foundational model dedicated to the domain of agriculture and livestock. First, we propose a large-scale dataset, named ALive, that leverages customized prompt generation strategy to overcome the scarcity of expert annotations. Our ALive dataset covers crops, livestock, and fishery, with around 600,000 image-text pairs. Second, we propose a training pipeline that integrates both contrastive and self-supervised learning to learn both global semantic and local fine-grained domain-specialized features. Experiments on diverse set of 20 downstream tasks demonstrate the effectiveness of AgriCLIP framework, achieving an absolute gain of 7.8\% in terms of average zero-shot classification accuracy, over the standard CLIP adaptation via domain-specialized ALive dataset. Our ALive dataset and code can be accessible at \href{https://github.com/umair1221/AgriCLIP/tree/main}{Github}.

==> Tables/abaltion_pre_trainings.tex <==
% \begin{table}[hbtp]
% \centering
% \caption{Experimental results for different combinations of CLIP + DINO}
% \label{tab:CLIP_DINO_Comb}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{CLIP (Def) + DINO (Def)}} & \multicolumn{2}{c}{\textbf{CLIP (PT) + DINO (Def)}} & \multicolumn{2}{c}{\textbf{CLIP (Def) + DINO (PT)}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%  & \textbf{50-50} & \textbf{70-30} & \textbf{50-50} & \textbf{70-30} & \textbf{50-50} & \textbf{70-30} \\
% \midrule
% \rowcolor{gray!10}
%  & & \textbf{Fish} & & & & \\
% \midrule
% Supermarket Fish \cite{ulucan2020large}   & 36.74 & 37.76 & 39.1 & 40.21 & 38.82 & 39.87 \\
% Aquarium Fish \cite{Aquarium28:online}   & 37.38 & 38.61 & 40.48 & 41.69 & 39.14 & 40.25 \\
% FishDataset \cite{FishData39:online}   & 42.71 & 43.88 & 46.28 & 47.52 & 44.76 & 46.03 \\
% DeepFish \cite{saleh2020realistic}  & \multicolumn{2}{c}{53.62} & \multicolumn{2}{c}{56.76} & \multicolumn{2}{c}{57.68} \\
% FishNet \cite{khan2023fishnet}  & 19.82 & 19.43 & 21.09 & 20.72 & 20.87 & 20.53 \\
% Fish Freshness \cite{Fresh}  & 53.02 & 54.24 & 55.04 & 56.27 & 54.57 & 55.68 \\
% Fish Species \cite{Specieclas87:online}  & 39.03 & 39.48 & 41.58 & 42.73 & 40.26 & 41.47 \\

% \midrule
% \rowcolor{gray!10}
% & & \textbf{Crops} & & & & \\
% \midrule
% Banana Deficiency \cite{sunitha2022images}  & 21.88 & 22.57 & 23.31 & 23.97 & 23.02 & 23.63 \\
% Soybean Weeds \cite{dosSantosFerreira2017weed}  & 55.99 & 57.33 & 58.47 & 59.83 & 57.94 & 59.18 \\
% Citrus Fruits \cite{sharif2018detection}& 34.58 & 38.04 & 37.02 & 40.38 & 36.79 & 40.23 \\
% Citrus Leaves \cite{sharif2018detection}& 35.77 & 36.93 & 38.12 & 39.19 & 37.87 & 39.04 \\
% Fruits Diseases \cite{kour2019plantaeK}  & 68.03 & 69.59 & 70.76 & 72.43 & 70.19 & 71.82 \\
% PlantDoc \cite{PlantDoc}  & 32.02 & 32.47 & 34.12 & 34.57 & 33.48 & 33.99 \\
% Wheat Rust \cite{YELLOWRU46:online}  & 58.16 & 59.30 & 64.32 & 63.68 & 61.45 & 62.59 \\
% Bean Lesion \cite{BeanLeaf6:online}  & 39.73 & 40.86 & 42.41 & 43.58 & 41.49 & 42.63 \\

% \midrule
% \rowcolor{gray!10}
% & & \textbf{Livestock} & & & & \\
%  \midrule
% Ovis-Aries \cite{abuJwade2023ovisAries} & 64.89 & 65.83 & 65.27 & 66.62 & 65.43 & 66.47 \\
% Cattle Breed \cite{CattleBr14:online} & 83.16 & 85.13 & 84.82 & 86.69 & 84.52 & 86.35 \\
% CID \cite{shagor2022cid} & 18.04 & 19.49 & 18.57 & 20.64 & 18.73 & 20.81 \\
% Horse \& Camel \cite{HORSESCA16:online} & 94.41 & 96.05 & 95.08 & 96.52 & 94.87 & 96.35 \\
% Animals-10 \cite{Animals176:online} & 96.82 & 95.87 & 98.55 & 98.36 & 97.36 & 96.89 \\
% \midrule
% \rowcolor{gray!10} % Adding a row color 
% \textbf{Average} & 49.28 & 50.31 & 51.55 & 52.61 & 50.96 & 52.07 \\
 
% \bottomrule
% \end{tabular}
% }
% \end{table}

% Updated with 70 only
\begin{table*}[hbtp]
\centering
\caption{Experimental results for different combinations of ${E}_{\text{img}}$ and ${E}^{S}_{\text{img}}$ encoders. Here, Def corresponds to using the encoder in its default state whereas PT refers to pre-trained on ALive dataset}
\label{tab:CLIP_DINO_Comb}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{CLIP (Def) + DINO (Def)} & \textbf{CLIP (PT) + DINO (Def)} & \textbf{CLIP (Def) + DINO (PT)} \\
\midrule
\rowcolor{gray!10}
 & \textbf{Fish} & & \\
\midrule
Supermarket Fish \cite{ulucan2020large}   & 37.76 & 40.21 & 39.87 \\
Aquarium Fish \cite{Aquarium28:online}   & 38.61 & 41.69 & 40.25 \\
FishDataset \cite{FishData39:online}   & 43.88 & 47.52 & 46.03 \\
DeepFish \cite{saleh2020realistic}  & 53.62 & 56.76 & 57.68 \\
FishNet \cite{khan2023fishnet}  & 19.43 & 20.72 & 20.53 \\
Fish Freshness \cite{Fresh}  & 54.24 & 56.27 & 55.68 \\
Fish Species \cite{Specieclas87:online}  & 39.48 & 42.73 & 41.47 \\

\midrule
\rowcolor{gray!10}
 & \textbf{Crops} & & \\
\midrule
Banana Deficiency \cite{sunitha2022images}  & 22.57 & 23.97 & 23.63 \\
Soybean Weeds \cite{dosSantosFerreira2017weed}  & 57.33 & 59.83 & 59.18 \\
Citrus Fruits \cite{sharif2018detection} & 38.04 & 40.38 & 40.23 \\
Citrus Leaves \cite{sharif2018detection} & 36.93 & 39.19 & 39.04 \\
Fruits Diseases \cite{kour2019plantaeK}  & 69.59 & 72.43 & 71.82 \\
PlantDoc \cite{PlantDoc}  & 32.47 & 34.57 & 33.99 \\
Wheat Rust \cite{YELLOWRU46:online}  & 59.30 & 63.68 & 62.59 \\
Bean Lesion \cite{BeanLeaf6:online}  & 40.86 & 43.58 & 42.63 \\

\midrule
\rowcolor{gray!10}
 & \textbf{Livestock} & & \\
 \midrule
Ovis-Aries \cite{abuJwade2023ovisAries} & 65.83 & 66.62 & 66.47 \\
Cattle Breed \cite{CattleBr14:online} & 85.13 & 86.69 & 86.35 \\
CID \cite{shagor2022cid} & 19.49 & 20.64 & 20.81 \\
Horse \& Camel \cite{HORSESCA16:online} & 96.05 & 96.52 & 96.35 \\
Animals-10 \cite{Animals176:online} & 95.87 & 98.36 & 96.89 \\
\midrule
\rowcolor{gray!10} % Adding a row color 
\textbf{Average} & 50.31 & 52.61 & 52.07 \\
 
\bottomrule
\end{tabular}
}
\end{table*}


==> Tables/data_composition.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|lccc}
    \toprule
         Type &  Tasks & Sensor &  Variabley & \#imgs  \\
         \midrule
          & Nutrients Deficiency \\
          & Weed Classification \\
           & Plant Disease Classification \\
           &  Fruits Classification  \\
           & Plant Specie Classification \\
           & Fish Abundance Classification  \\ 
           & Cattle Breed Recognition \\
           & Horse Classification \\
         \midrule
         Total  \\
         \bottomrule
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> Tables/main_table1.tex <==
\begin{table*}[htbp]
\centering
\caption{Performance of CLIP models across different configurations and data splits, categorized by dataset types.}
\label{tab:CLIP-performance}
\resizebox{0.6\textwidth}{!}{%
\begin{tabularx}{\textwidth}{>{\hsize=0.9\hsize}X *{6}{>{\centering\arraybackslash\hsize=0.3\hsize}X}}

\toprule
\rowcolor{gray!30}  % Adds a grey background to the header row for emphasis
\textbf{Dataset} & \multicolumn{2}{c}{\textbf{Default CLIP}} & \multicolumn{2}{c}{\textbf{PT CLIP}} & \multicolumn{2}{c}{\textbf{PT CLIP + CP}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& \textbf{50-50} & \textbf{70-30} & \textbf{50-50} & \textbf{70-30} & \textbf{50-50} & \textbf{70-30} \\
\midrule
\rowcolor{gray!10}
 & & & \textbf{Fish} & & & \\
\midrule
Supermarket Fish \cite{ulucan2020large}   & 1.39 & 1.66 & 20.48 & 22.57 & 20.93 & 23.45 \\
Aquarium Fish \cite{Aquarium28:online}  & 24   & 22.85 & 29.62 & 27.13 & 30.17 & 27.65 \\
FishDataset \cite{FishData39:online} & 16.37 & 16.04 & 33.54 & 32.47 & 34.22 & 33.18 \\
DeepFish \cite{saleh2020realistic}  & \multicolumn{2}{c}{45.41} & \multicolumn{2}{c}{55.96} & \multicolumn{2}{c}{56.44} \\
FishNet \cite{khan2023fishnet}  & 0.14 & 0.15 & 17.39 & 19.52 & 18.76 & 20.83 \\
Fish Freshness \cite{Fresh}  & 28.15 & 29.37 & 48.92 & 50.05 & 49.80 & 51.25 \\
Fish Species \cite{Specieclas87:online}  & 12.44 & 13.68 & 34.57 & 35.89 & 35.22 & 36.54 \\
\midrule
\rowcolor{gray!10}
 & & & \textbf{Crops} & & & \\
\midrule
Banana Deficiency \cite{sunitha2022images}  & 10.95 & 14.08 & 16.88 & 15.64 & 17.15 & 16.24 \\
Soybean Weeds \cite{dosSantosFerreira2017weed}  & 32.38 & 41.4 & 56.37 & 58.92 & 56.81 & 59.27 \\
Citrus Fruits \cite{sharif2018detection} & 11.24 & 38.09 & 35.16 & 39.55 & 35.68 & 37.81 \\
Citrus Leaves \cite{sharif2018detection} & 10.16 & 2.18 & 26.84 & 23.97 & 27.25 & 24.39 \\
Fruits Diseases \cite{kour2019plantaeK}  & 75.95 & 68.9 & 70.44 & 73.26 & 70.98 & 72.01 \\
PlantDoc \cite{PlantDoc}  & 6.77  & 6.02 & 27.69 & 29.18 & 29.86 & 31.72 \\
Wheat Rust \cite{YELLOWRU46:online}  & 33.42 & 34.11 & 51.39 & 53.45 & 52.67 & 54.82 \\
Bean Lesion \cite{BeanLeaf6:online}  & 17.89 & 18.73 & 36.56 & 38.47 & 37.44 & 39.58 \\
\midrule
\rowcolor{gray!10}
 & & & \textbf{LiveStock} & & & \\
\midrule
Ovis-Aries \cite{abuJwade2023ovisAries} & 38.81 & 39.52 & 56.28 & 58.37 & 57.18 & 59.24 \\
Cattle Breed \cite{CattleBr14:online} & 60.02 & 61.67 & 74.82 & 76.94 & 75.22 & 77.38 \\
CID \cite{shagor2022cid} & 04.87  & 05.62  & 16.34 & 17.52 & 18.05 & 19.28 \\
Horse \& Camel \cite{HORSESCA16:online} & 88.27 & 89.13 & 90.79 & 92.23 & 91.65 & 93.08 \\
Animals-10 \cite{Animals176:online} & 94.36 & 95.48 & 95.83 & 97.12 & 96.74 & 97.95 \\

\bottomrule

\rowcolor{gray!20} % Adding a row for averages
\textbf{Average} & 30.64 & 32.16 & 44.78 & 45.90 & 45.60 & 46.59 \\

\bottomrule
\end{tabularx}
}
\end{table*}

==> Tables/main_table2.tex <==
\begin{table*}[htbp]
\centering
\caption{Performance of various configurations of CLIP and DINO across different data splits.}
\label{tab:CLIP+DINO-performance}
\resizebox{1\textwidth}{!}{ % Resizes the table to fit the width of the text area
\begin{tabular}{lcccccccc}
\toprule
\rowcolor{gray!30}
Dataset & \multicolumn{2}{c}{CLIP (Def) + DINO (Def)} & \multicolumn{2}{c}{CLIP (PT) + DINO (Def)} & \multicolumn{2}{c}{CLIP (Def) + DINO (PT)} & \multicolumn{2}{c}{CLIP (PT) + DINO (PT)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & 50-50 & 70-30 & 50-50 & 70-30 & 50-50 & 70-30 & 50-50 & 70-30 \\
\midrule
\rowcolor{gray!10}
 & & & & \textbf{Fish} & & & & \\
\midrule
Supermarket Fish \cite{ulucan2020large}   & 36.74 & 37.76 & 39.1 & 40.21 & 38.82 & 39.87 & 40.25 & 41.38 \\
Aquarium Fish \cite{Aquarium28:online}   & 37.38 & 38.61 & 40.48 & 41.69 & 39.14 & 40.25 & 41.89 & 43.06 \\
FishDataset \cite{FishData39:online}   & 42.71 & 43.88 & 46.28 & 47.52 & 44.76 & 46.03 & 47.96 & 49.23 \\
DeepFish \cite{saleh2020realistic}  & \multicolumn{2}{c}{53.62} & \multicolumn{2}{c}{56.76} & \multicolumn{2}{c}{57.68} & \multicolumn{2}{c}{57.78} \\
FishNet \cite{khan2023fishnet}  & 19.82 & 19.43 & 21.09 & 20.72 & 20.87 & 20.53 & 21.97 & 21.58 \\
Fish Freshness \cite{Fresh}  & 53.02 & 54.24 & 55.04 & 56.27 & 54.57 & 55.68 & 56.59 & 57.75 \\
Fish Species \cite{Specieclas87:online}  & 39.03 & 39.48 & 41.58 & 42.73 & 40.26 & 41.47 & 43.05 & 44.21 \\
\midrule
\rowcolor{gray!10}
 & & & & \textbf{Crops} & & & & \\
\midrule
Banana Deficiency \cite{sunitha2022images}  & 21.88 & 22.57 & 23.31 & 23.97 & 23.02 & 23.63 & 23.91 & 24.57 \\
Soybean Weeds \cite{dosSantosFerreira2017weed}  & 55.99 & 57.33 & 58.47 & 59.83 & 57.94 & 59.18 & 59.56 & 60.88 \\
Citrus Fruits \cite{sharif2018detection}& 34.58 & 38.04 & 37.02 & 40.38 & 36.79 & 40.23 & 38.24 & 40.21 \\
Citrus Leaves \cite{sharif2018detection}& 35.77 & 36.93 & 38.12 & 39.19 & 37.87 & 39.04 & 39.09 & 40.27 \\
Fruits Diseases \cite{kour2019plantaeK}  & 68.03 & 69.59 & 70.76 & 72.43 & 70.19 & 71.82 & 75.36 & 73.98 \\
PlantDoc \cite{PlantDoc}  & 32.02 & 32.47 & 34.12 & 34.57 & 33.48 & 33.99 & 34.96 & 35.42 \\
Wheat Rust \cite{YELLOWRU46:online}  & 58.16 & 59.30 & 64.32 & 63.68 & 61.45 & 62.59 & 66.16 & 67.38 \\
Bean Lesion \cite{BeanLeaf6:online}  & 39.73 & 40.86 & 42.41 & 43.58 & 41.49 & 42.63 & 44.15 & 44.98 \\
\midrule
\rowcolor{gray!10}
 & & & & \textbf{LiveStock} & & & & \\
 \midrule
Ovis-Aries \cite{abuJwade2023ovisAries} & 64.89 & 65.83 & 65.27 & 66.62 & 65.43 & 66.47 & 66.68 & 67.29 \\
Cattle Breed \cite{CattleBr14:online} & 83.16 & 85.13 & 84.82 & 86.69 & 84.52 & 86.35 & 85.23 & 86.85 \\
CID \cite{shagor2022cid} & 18.04 & 19.49 & 18.57 & 20.64 & 18.73 & 20.81 & 19.34 & 21.14 \\
Horse \& Camel \cite{HORSESCA16:online} & 94.41 & 96.05 & 95.08 & 96.52 & 94.87 & 96.35 & 95.78 & 97.62 \\
Animals-10 \cite{Animals176:online} & 96.82 & 95.87 & 98.55 & 98.36 & 97.36 & 96.89 & 98.27 & 99.50 \\
\midrule
\rowcolor{gray!10} % Adding a row color 
\textbf{Average} & 49.28 & 50.31 & 51.55 & 52.61 & 50.96 & 52.07 & 52.81 & 53.75 \\
 
\bottomrule
\end{tabular}
}
\end{table*}

==> junk.tex <==
% \noindent\textbf{Implications for Agricultural AI}
% The findings from this study have significant implications for the deployment of AI technologies in agriculture. By enhancing the accuracy and reliability of such models, farmers and agricultural scientists can better utilize these tools for precision agriculture, crop monitoring, and disease detection. It can also be integrated into visual question-answering (VQA) systems where farmers can interact with the large language models to answer their queries. This could lead to more informed decision-making and, ultimately, more sustainable agricultural practices.

% \noindent\textbf{Future Work}
% Future research should explore the scalability of these approaches to other types of environmental and biological data within agriculture and beyond. Further experimentations could also examine the robustness of these models against variations in data quality and real-world conditions. Additionally, integrating these models into real-time decision-making systems could be a valuable direction, providing actionable insights directly into the field.


% \subsection{Ablation Study}
% For the ablation study, two experiments are conducted to assess different aspects of the methodology, which involves the curated dataset and the DINO model. 

% To determine the optimal model configuration, we conducted a series of experiments using different combinations of CLIP and DINO, both in their pre-trained state and with default weights. We evaluated each combination on our downstream datasets to identify the best-performing setup. Our experiments revealed that combining both models in their pre-trained condition yielded the highest classification accuracy across all datasets. This finding highlights the importance of pre-training and feature alignment in achieving state-of-the-art performance in agricultural zero-shot classification
